StylePTB: A Compositional Benchmark for Fine-grained Controllable Text Style Transfer

Text style transfer aims to controllably generate text with targeted stylistic changes while maintaining core meaning from the source sentence constant. Many of the existing style transfer benchmarks primarily focus on individual high-level semantic changes (e.g. positive to negative), which enable controllability at a high level but do not offer fine-grained control involving sentence structure, emphasis, and content of the sentence. In this paper, we introduce a large-scale benchmark, StylePTB, with (1) paired sentences undergoing 21 fine-grained stylistic changes spanning atomic lexical, syntactic, semantic, and thematic transfers of text, as well as (2) compositions of multiple transfers which allow modeling of fine-grained stylistic changes as building blocks for more complex, high-level transfers. By benchmarking existing methods on StylePTB, we find that they struggle to model fine-grained changes and have an even more difficult time composing multiple styles. As a result, StylePTB brings novel challenges that we hope will encourage future research in controllable text style transfer, compositional models, and learning disentangled representations. Solving these challenges would present important steps towards controllable text generation.

==> NAACL2021_Disentangling Text/figs/overview.tex <==
\begin{figure}[tbp]
\centering
\vspace{-0mm}
\includegraphics[width=\linewidth]{figs/overview_fig.pdf}
\vspace{-4mm}
\caption{\datashort\ provides a large-scale resource to study \textit{fine-grained compositional style transfer}. The styles provided in \datashort\ (in \textbf{\color{gg}{green}}\color{black}) span lexical, syntax, semantic, and thematic aspects~\cite{dimarco1993computational} which can be composed to form high-level style transfers as commonly studied in existing benchmarks (\textit{e.g.} Yelp for sentiment~\cite{shen2017style} and GYAFC for formality~\cite{rao2018dear}).\vspace{-2mm}}
\label{overview_fig}
\end{figure}
% The two sentiment transfer examples came from Yelp dataset and the two formality transfer came from GYAFC E\&M. 
% \datashort\ provides resources to study \textit{fine-grained compositional style transfer}. The styles provided in \datashort\ (in green) can be composed to form high-level style transforms as commonly studied in existing benchmarks (e.g. negative to positive, informal to formal).\vspace{-4mm}}

==> NAACL2021_Disentangling Text/tables/amttransfer.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.0pt}
\centering
\footnotesize
\begin{tabular}{llcccccc}
\Xhline{3\arrayrulewidth}
\multicolumn{2}{l}{Human annotated Tasks} & \multicolumn{1}{l}{total tasks} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}tasks rejected \\ and republished\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}tasks with "N/A" \\ or not-make-sense\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}total sentences\\ added to dataset\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Price per task\\ (in USD)\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Number of\\ Unique workers\end{tabular}} \\ \hline
Semantics & \begin{tabular}[c]{@{}l@{}}Information\\ Addition\end{tabular} & $4412$ & $17$ & $2296$ & $2114$ & $0.07$ & $19$ \\ \hline
\multirow{2}{*}{Thematics} & ADJ emphasis & $808$ & $14$ & $112$ & $696$ & $0.13$ & $9$ \\ 
 & Verb emphasis & $1373$ & $141$ & $172$ & $1201$ & $0.12$ & $13$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{\label{tab:amt}Statistics on the collection of data in three transfers using  human annotation on AMT.\vspace{-4mm}}
\end{table*}

==> NAACL2021_Disentangling Text/tables/autotransfer.tex <==
\begin{table}[]
\centering
\footnotesize
\centering
\begin{tabular}{llc}
% \hline % nothing precedes \multicolumn
%\multicolumn{2}{l}{Automated Transformations}                                                                                                                              & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}parallel pairs\\ of sentences\end{tabular}} \\ 
\Xhline{3\arrayrulewidth}
Category & Transfer & Number \\
\Xhline{0.5\arrayrulewidth}
\multirow{10}{*}{Lexical}                                                                      & Noun synonym replacement                                                     & $5948$                                                                                          \\ 
% \cline{2-3} 
                                                                                              & Noun antonym replacement                                                     & $2227$                                                                                          \\ 
                                                                                            %   \cline{2-3} 
                                                                                              & Verb synonym replacement                                                     & $2574$                                                                                           \\ 
                                                                                            %   \cline{2-3} 
                                                                                              & Verb antonym replacement                                                     & $1284$                                                                                          \\ 
                                                                                            %   \cline{2-3} 
                                                                                              & ADJ synonym replacement                                                      & $434$                                                                                           \\ 
                                                                                            %   \cline{2-3} 
                                                                                              & ADJ antonym replacement                                                      & $1146$                                                                                          \\ 
                                                                                            %   \cline{2-3} 
                                                                                              & \begin{tabular}[c]{@{}l@{}}Most frequent synonym\\ replacement\end{tabular}  & $4722$                                                                                          \\ 
                                                                                            %   \cline{2-3} 
                                                                                              & \begin{tabular}[c]{@{}l@{}}Least frequent synonym\\ replacement\end{tabular} & $7112$                                                                                          \\ \hline
\multirow{5}{*}{Syntax}                                                                       & To future tense                                                              & $7272$                                                                                          \\ 
% \cline{2-3} 
                                                                                              & To present tense                                                             & $4365$                                                                                          \\ 
                                                                                            %   \cline{2-3} 
                                                                                              & To past tense                                                                & $4422$                                                                                          \\ 
                                                                                            %   \cline{2-3} 
                                                                                              %& Active to Passive                                                            & $2737$                                                                                          \\ 
                                                                                            %   \cline{2-3} 
                                                                                              %& Passive to active                                                            & $71$                                                                                            \\ 
                                                                                            %   \cline{2-3} 
                                               & Active $\leftrightarrow$ passive & $2808$ \\
                                               & PP front $\leftrightarrow$ back & $467$ \\  
                                               %& PP front to back                                                             & $460$                                                                                           \\ 
                                                                                            %   \cline{2-3} 
                                                                                              %& PP back to front                                                             & $7$                                                                                             \\
                                                                                              \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Semantics\\ (information\\ deletion)\end{tabular}} & ADJ or ADV removal                                                           & $4863$                                                                                          \\ 
% \cline{2-3} 
& PP removal & $4767$ \\ 
                                                                                            %   \cline{2-3} 
                                                                                              & Substatement removal                                                         & $1345$                                                                                          \\ 
                                                                                            %   \hline
                                                                                            %  \Xhline{3\arrayrulewidth}
& Information Addition & $2114$ \\
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Thematic \end{tabular}} & Verb/action emphasis                                                           & $1201$                                                                                          \\ 
% \cline{2-3} 
                                                                                              & Adj emphasis                                                                   & $696$                                                                                          \\ 
                                                                                            %   \cline{2-3} 

                                                                                            %   \hline
                                                                                             \Xhline{3\arrayrulewidth}
\end{tabular}
\caption{\datashort\ is a large-scale resource spanning $59,767$ sentence pairs  across $21$ individual styles.\vspace{-2mm}}
\label{tab:aut}
\end{table}

==> NAACL2021_Disentangling Text/tables/baselineresults.tex <==
\footnotesize
\begin{tabular}{|l|l|r|r|r|r|r|r|r|}
\hline
Baseline Model & Transformation & \multicolumn{1}{l|}{BLEU-1} & \multicolumn{1}{l|}{BLEU-2} & \multicolumn{1}{l|}{BLEU-3} & \multicolumn{1}{l|}{BLEU-4} & \multicolumn{1}{l|}{METEOR} & \multicolumn{1}{l|}{ROUGE\_L} & \multicolumn{1}{l|}{CiDER} \\ \hline
\multirow{13}{*}{GPT Baseline} & To Future Tense & 0.8954 & 0.8519 & 0.8127 & 0.7776 & 0.5399 & 0.8987 & 7.7087 \\ \cline{2-9} 
 & To Present Tense & 0.8357 & 0.7762 & 0.7219 & 0.6738 & 0.484 & 0.8422 & 6.6996 \\ \cline{2-9} 
 & To Past tense & 0.7539 & 0.6625 & 0.5862 & 0.5237 & 0.4121 & 0.7722 & 5.2932 \\ \cline{2-9} 
 & Active to Passive & 0.4756 & 0.3293 & 0.2382 & 0.189 & 0.216 & 0.4635 & 1.8209 \\ \cline{2-9} 
 & Passive to active & 0.4325 & 0.2709 & 0.1672 & 0.1203 & 0.1908 & 0.4344 & 1.3287 \\ \cline{2-9} 
 & PP Front to Back & 0.3976 & 0.2095 & 0.0808 & 0.0006 & 0.1836 & 0.4057 & 0.886 \\ \cline{2-9} 
 & PP back to Front & 0.4065 & 0.2413 & 0.0912 & 0.0007 & 0.1659 & 0.4061 & 0.9306 \\ \cline{2-9} 
 & ADJ or ADV Removal & 0.6471 & 0.508 & 0.3941 & 0.3084 & 0.3125 & 0.6523 & 3.2589 \\ \cline{2-9} 
 & PP Removal & 0.7631 & 0.7004 & 0.6451 & 0.593 & 0.4192 & 0.7867 & 6.0119 \\ \cline{2-9} 
 & Substatement Removal & 0.4303 & 0.3316 & 0.2474 & 0.1757 & 0.2498 & 0.5881 & 3.0894 \\ \cline{2-9} 
 & Information Addition & 0.4793 & 0.3048 & 0.1891 & 0.1205 & 0.2074 & 0.4746 & 1.3588 \\ \cline{2-9} 
 & Adjective Emphasis & 0.2629 & 0.0793 & 0.0282 & 0.0003 & 0.1122 & 0.1884 & 0.3863 \\ \cline{2-9} 
 & Verb/Action Emphasis & 0.3087 & 0.1697 & 0.0949 & 0.0405 & 0.1399 & 0.2921 & 0.5925 \\ \hline
\multirow{13}{*}{GRU attn} & To Future Tense & 0.5271 & 0.3675 & 0.2609 & 0.1884 & 0.1727 & 0.5309 & 1.5253 \\ \cline{2-9} 
 & To Present Tense & 0.4784 & 0.3129 & 0.2043 & 0.1328 & 0.1552 & 0.4898 & 1.3735 \\ \cline{2-9} 
 & To Past tense & 0.516 & 0.3605 & 0.2674 & 0.2101 & 0.1899 & 0.5178 & 1.8185 \\ \cline{2-9} 
 & Active to Passive & 0.3725 & 0.2199 & 0.1414 & 0.103 & 0.1308 & 0.3451 & 0.8446 \\ \cline{2-9} 
 & Passive to active & 0.3394 & 0.2137 & 0.16 & 0.1315 & 0.1262 & 0.3314 & 1.0615 \\ \cline{2-9} 
 & PP Front to Back & 0.3928 & 0.2802 & 0.2071 & 0.1607 & 0.1618 & 0.3914 & 1.4918 \\ \cline{2-9} 
 & PP back to Front & 0.2978 & 0.1572 & 0.0904 & 0.0595 & 0.1123 & 0.2836 & 0.6057 \\ \cline{2-9} 
 & ADJ or ADV Removal & 0.4497 & 0.2735 & 0.1723 & 0.1118 & 0.1398 & 0.4688 & 1.1711 \\ \cline{2-9} 
 & PP Removal & 0.3303 & 0.1949 & 0.1212 & 0.0814 & 0.1124 & 0.3634 & 1.0036 \\ \cline{2-9} 
 & Substatement Removal & 0.3165 & 0.1924 & 0.1096 & 0.0009 & 0.1004 & 0.3678 & 1.0409 \\ \cline{2-9} 
 & Information Addition & 0.345 & 0.1804 & 0.094 & 0.0527 & 0.0983 & 0.335 & 0.6315 \\ \cline{2-9} 
 & Adjective Emphasis & 0.1873 & 0.0581 & 0.0184 & 0.0002 & 0.0593 & 0.1794 & 0.1414 \\ \cline{2-9} 
 & Verb/Action Emphasis & 0.2885 & 0.1268 & 0.0656 & 0.0379 & 0.0982 & 0.2748 & 0.3003 \\ \hline
\multirow{13}{*}{RetrieveEdit} & To Future Tense & 0.8992 & 0.8536 & 0.8145 & 0.7783 & 0.531 & 0.9013 & 7.7309 \\ \cline{2-9} 
 & To Present Tense & 0.9352 & 0.9031 & 0.8731 & 0.8474 & 0.6062 & 0.9328 & 8.3577 \\ \cline{2-9} 
 & To Past tense & 0.9094 & 0.8702 & 0.8302 & 0.7926 & 0.5986 & 0.9156 & 7.9874 \\ \cline{2-9} 
 & Active to Passive & 0.6809 & 0.5981 & 0.5031 & 0.4273 & 0.3827 & 0.6629 & 4.5351 \\ \cline{2-9} 
 & Passive to active & 0.7143 & 0.6587 & 0.5592 & 0.4744 & 0.397 & 0.7317 & 5.024 \\ \cline{2-9} 
 & PP Front to Back & 0.5408 & 0.4226 & 0.3009 & 0.1763 & 0.2474 & 0.5474 & 2.5362 \\ \cline{2-9} 
 & PP back to Front & 0.6486 & 0.5842 & 0.5353 & 0.4914 & 0.3333 & 0.6563 & 4.6667 \\ \cline{2-9} 
 & ADJ or ADV Removal & 0.8972 & 0.8408 & 0.7855 & 0.7307 & 0.5109 & 0.9185 & 7.4607 \\ \cline{2-9} 
 & PP Removal & 0.798 & 0.7704 & 0.7392 & 0.7117 & 0.4778 & 0.8455 & 7.1105 \\ \cline{2-9} 
 & Substatement Removal & 0.7056 & 0.6783 & 0.6474 & 0.6068 & 0.4053 & 0.7671 & 6.183 \\ \cline{2-9} 
 & Information Addition & 0.4928 & 0.3959 & 0.3282 & 0.2746 & 0.2841 & 0.6028 & 3.4011 \\ \cline{2-9} 
 & Adjective Emphasis & 0.3866 & 0.276 & 0.2106 & 0.1637 & 0.1933 & 0.369 & 1.6793 \\ \cline{2-9} 
 & Verb/Action Emphasis & 0.4162 & 0.2844 & 0.2091 & 0.1483 & 0.2229 & 0.4234 & 1.7782 \\ \hline
\end{tabular}

==> NAACL2021_Disentangling Text/tables/bertdist.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{6.0pt}
\centering
\footnotesize
\begin{tabular}{lcc}
\Xhline{3\arrayrulewidth}
Transfer & MSE \textcolor{gg}{$\downarrow$} & Cosine \textcolor{gg}{$\uparrow$} \\ \hline
To Future Tense & 0.015 & 0.978 \\
To Past Tense & 0.019 & 0.971 \\
To Present Tense & 0.012 & 0.982 \\
Active To Passive & 0.018 & 0.973 \\
Passive To Active & 0.029 & 0.960 \\
PP Front to Back & 0.021 & 0.969 \\
PP Back To Front & 0.016 & 0.977 \\
ADJ or ADV Removal & 0.013 & 0.981 \\
PP Removal & 0.032 & 0.953 \\
Substatement Removal & 0.045 & 0.934 \\
Information Addition & 0.012 & 0.981 \\
Adjective Emphasis & 0.031 & 0.952 \\
Verb/Action Emphasis & 0.035 & 0.948 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{\label{tab:bertd} Average $\ell_2$ distance and cosine similarity between BERT pooled output vectors of original and transferred sentences of the syntax, semantic and thematic transfers.\vspace{-4mm}}
\end{table}

==> NAACL2021_Disentangling Text/tables/biasexample.tex <==
\begin{table}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{ll}
\Xhline{3\arrayrulewidth}

% \begin{table}[]
% \begin{tabular}{ll}
Text Generated by \textsc{GPT2} & Text after occupation replacement \\ \hline
\begin{tabular}[c]{@{}l@{}}The man worked as a \textbf{security guard}\\ for the family's hotel until the weekend.\end{tabular} & \begin{tabular}[c]{@{}l@{}}The man worked as a \textbf{receptionist}\\ for the family's hotel until the weekend.\end{tabular} \\
The man worked as a driver for his father. & The man worked as a \textbf{personal care aide} for his father. \\
\begin{tabular}[c]{@{}l@{}}The woman worked as a \textbf{maid} at a\\ resort in a small town.\end{tabular} & \begin{tabular}[c]{@{}l@{}}The woman worked as a \textbf{driver} at a resort\\ in a small town.\end{tabular} \\
The woman worked as a \textbf{nurse} at a facility. & The woman worked as a \textbf{construction worker} at a facility. \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Examples of sentences generated by \textsc{GPT2} and with occupation replacements that are rated as ``Significantly Less Biased'' after the change by human annotators. \vspace{-4mm}}
\label{last_bias_example}
\end{table}

==> NAACL2021_Disentangling Text/tables/biasexperimenttable.tex <==
\begin{table}[]
\fontsize{9}{11}\selectfont
\centering

\setlength\tabcolsep{3.5pt}

\begin{tabular}{l |cc|c}
\Xhline{3\arrayrulewidth}
& Male context & Female context & Total \\ \hline
Biased & $21$ & $28$ & $49$ \\
Not Biased & $29$ & $22$ & $51$  \\ \hline
Total & $50$ & $50$ & $100$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Category & Number \\
\Xhline{0.5\arrayrulewidth}
Significantly more biased & $0$ \\
Slightly more biased & $0$ \\
Little or no change in bias & $22$ \\
Slightly less biased & $5$ \\
Significantly less biased & $\mathbf{22}$ \\ \hline
Total & $49$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{-0mm}
\caption{\textbf{Top table:} Human annotators found that $21$ out of $50$ sentences generated by \textsc{GPT2} on ``The man worked as'' and $28$ out of $50$ sentences generated by \textsc{GPT2} on ``The woman worked as'' to exhibit gender bias. \textbf{Bottom table:} Out of the $49$ biased sentences, after using style transfer to replace occupations with randomly sampled ones, human annotators found that $22$ of them are significantly less biased while the rest are either slightly less biased or neutral. \vspace{-2mm}}
\label{biasexperiment}
\end{table}

==> NAACL2021_Disentangling Text/tables/comp_full.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.0pt}
\centering
\footnotesize
\begin{tabular}{lllccccccc}
\Xhline{3\arrayrulewidth}
Dataset & Transfers & Model & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & METEOR & ROUGE\_L & CiDER \\ \hline
\multirow{18}{*}{\begin{tabular}[c]{@{}l@{}}Tense\\ +\\ Voice\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToPast+\\ ActiveToPassive\end{tabular}} & \textsc{SeqGPT} & 0.332 & 0.155 & 0.057 & 0.024 & 0.144 & 0.300 & 0.636 \\
 & & \textsc{\modelshort-zero} & 0.337 & 0.163 & 0.075 & 0.029 & 0.154 & 0.283 & 0.760 \\
 & & \modelshort & \textbf{0.409} & \textbf{0.238} & \textbf{0.133} & \textbf{0.064} & \textbf{0.180} & \textbf{0.378} & \textbf{1.029} \\
 \cline{2-10}
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToFuture+\\ ActiveToPassive\end{tabular}} & \textsc{SeqGPT} & 0.391 & 0.222 & 0.120 & 0.065 & 0.167 & 0.373 & 0.866 \\
 & & \textsc{\modelshort-zero} & 0.419 & 0.243 & 0.114 & 0.047 & 0.209 & 0.325 & 1.238 \\
 & & \modelshort & \textbf{0.496} & \textbf{0.340} & \textbf{0.240} & \textbf{0.185} & \textbf{0.217} & \textbf{0.479} & \textbf{1.800} \\
 \cline{2-10}
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToFuture+\\ PassiveToActive\end{tabular}} & \textsc{SeqGPT} & 0.401 & 0.212 & 0.097 & 0.048 & 0.163 & 0.385 & 0.888 \\
 & & \textsc{\modelshort-zero} & 0.399 & 0.245 & 0.123 & 0.047 & 0.212 & 0.349 & 1.075 \\ 
 & & \modelshort & \textbf{0.528} & \textbf{0.364} & \textbf{0.259} & \textbf{0.197} & \textbf{0.234} & \textbf{0.524} & \textbf{2.020} \\
 \cline{2-10}
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToPast+\\ PassiveToActive\end{tabular}} & \textsc{SeqGPT} & 0.381 & 0.210 & 0.098 & 0.045 & 0.156 & 0.368 & 0.876 \\
 & & \textsc{\modelshort-zero} & 0.365 & 0.181 & 0.073 & 0.025 & 0.156 & 0.343 & 0.752 \\ 
 & & \modelshort & \textbf{0.474} & \textbf{0.297} & \textbf{0.175} & \textbf{0.099} & \textbf{0.206} & \textbf{0.473} & \textbf{1.513} \\
 \cline{2-10} 
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToPresent+\\ PassiveToActive\end{tabular}} & \textsc{SeqGPT} & 0.348 & 0.189 & 0.085 & 0.037 & 0.142 & 0.343 & 0.745 \\
 & & \textsc{\modelshort-zero} & 0.424 & 0.257 & 0.118 & 0.046 & 0.208 & 0.389 & 1.025 \\
 & & \modelshort & \textbf{0.523} & \textbf{0.366} & \textbf{0.264} & \textbf{0.210} & \textbf{0.243} & \textbf{0.522} & \textbf{2.118} \\
 \cline{2-10} 
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToPresent+\\ ActiveToPassive\end{tabular}} & \textsc{SeqGPT} & 0.396 & 0.256 & 0.177 & 0.136 & 0.179 & 0.384 & 1.209 \\
 & & \textsc{\modelshort-zero} & 0.445 & 0.254 & 0.120 & 0.059 & 0.212 & 0.348 & 1.271 \\
 & & \modelshort & \textbf{0.503} & \textbf{0.358} & \textbf{0.271} & \textbf{0.223} & \textbf{0.233} & \textbf{0.491} & \textbf{2.118} \\
 \hline
 \multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Tense\\ +\\ PP \\ Removal\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToFuture+\\ PPRemoval\end{tabular}} & \textsc{SeqGPT} & 0.722 & 0.644 & \textbf{0.581} & \textbf{0.524} & 0.385 & \textbf{0.755} & 5.562 \\
 & & \textsc{\modelshort-zero} & 0.465 & 0.335 & 0.221 & 0.137 & 0.313 & 0.496 & 1.907 \\
 & & \modelshort & \textbf{0.738} & \textbf{0.652} & 0.578 & 0.518 & \textbf{0.393} & 0.755 & \textbf{5.289} \\
 \cline{2-10} 
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToPast+\\ PPRemoval\end{tabular}} & \textsc{SeqGPT} & 0.714 & 0.640 & 0.573 & 0.510 & 0.374 & 0.724 & 5.152 \\
 & & \textsc{\modelshort-zero} & 0.542 & 0.389 & 0.268 & 0.182 & 0.314 & 0.535 & 2.103 \\
 & & \modelshort & \textbf{0.772} & \textbf{0.695} & \textbf{0.624} & \textbf{0.564} & \textbf{0.421} & \textbf{0.775} & \textbf{5.585} \\
 \cline{2-10} 
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToPresent+\\ PPRemoval\end{tabular}} & \textsc{SeqGPT} & 0.618 & 0.518 & 0.435 & 0.368 & 0.338 & 0.663 & 4.119 \\
 & & \textsc{\modelshort-zero} & 0.545 & 0.393 & 0.269 & 0.184 & 0.323 & 0.539 & 2.017 \\
 & & \modelshort & \textbf{0.709} & \textbf{0.609} & \textbf{0.523} & \textbf{0.446} & \textbf{0.718} & \textbf{0.718} & \textbf{4.588} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on compositions of transfers using sequentially applying \textsc{GPT2} (\textsc{SeqGPT}), \textsc{\modelshort-zero} (adding compositional model but not compositional data) and \modelshort\ (with both compositional model and data). The result shows that \modelshort\ significantly outperforms the other two methods, and zero-shot remains challenging as \textsc{\modelshort-zero} does not perform very well in comparison. \vspace{-4mm}}
\label{tab:comp_full}
\end{table*}

==> NAACL2021_Disentangling Text/tables/comp_short.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transfers & Model & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & METEOR & ROUGE\_L & CiDER \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToFuture+\\ ActiveToPassive\end{tabular}}  & \textsc{GPT2} & 0.391 & 0.222 & 0.120 & 0.065 & 0.167 & 0.373 & 0.866 \\
& \textsc{\modelshort-zero} & 0.419 & 0.243 & 0.114 & 0.047 & 0.209 & 0.325 & 1.238 \\
& \modelshort & \textbf{0.496} & \textbf{0.340} & \textbf{0.240} & \textbf{0.185} & \textbf{0.217} & \textbf{0.479} & \textbf{1.800} \\
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ToPast+\\ PPRemoval\end{tabular}} & \textsc{GPT2} & 0.714 & 0.640 & 0.573 & 0.510 & 0.374 & 0.724 & 5.152 \\
& \textsc{\modelshort-zero} & 0.542 & 0.389 & 0.268 & 0.182 & 0.314 & 0.535 & 2.103 \\
& \modelshort & \textbf{0.772} & \textbf{0.695} & \textbf{0.624} & \textbf{0.564} & \textbf{0.421} & \textbf{0.775} & \textbf{5.585} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on compositions of transfers: \modelshort\ with compositional data works better than \textsc{\modelshort-zero} (without compositional data), and sequentially applying \textsc{GPT2} models.\vspace{-2mm}}
\label{tab:comp_short}
\end{table*}

==> NAACL2021_Disentangling Text/tables/composeexample.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\begin{tabular}{l|l|l}
\Xhline{3\arrayrulewidth}
Transfer & To Future + Passive To Active & To Past + PP Removal \\ \hline
Source Sentence & \begin{tabular}[c]{@{}l@{}}NUM \% was risen by sales to NUM billion from NUM billion\end{tabular} & \begin{tabular}[c]{@{}l@{}}the bond market was unmoved\\ by the economic statistics\end{tabular} \\ \hline
Target Sentence & sales will rise NUM \% to NUM billion from NUM billion & the bond market is unmoved \\ \hline
\textsc{SeqGPT} & willalesalesalesales to billion from from NUM billion & the bond market is is \\ \hline
\textsc{\modelshort-zero} & \begin{tabular}[c]{@{}l@{}}NUM \% \% \% risen risen sales \\ sales NUM NUM from NUM billion\end{tabular} & \begin{tabular}[c]{@{}l@{}}the bond market is unmoved\\ by the economic statistics\end{tabular} \\
\hline
\modelshort & {\color{gg}sales will rise NUM \% to NUM billion from NUM billion} & {\color{gg}the bond market is unmoved} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{2 examples of composition transfers generated by \modelshort, \textsc{SeqGPT} and \textsc{\modelshort-zero}. \modelshort \ successfully models compositional transfers across multiple styles.\vspace{-4mm}}
\label{tab:comp_example_supp}
\end{table*}

==> NAACL2021_Disentangling Text/tables/composeexample_short.tex <==
\definecolor{gg}{RGB}{15,150,15}
\definecolor{rr}{RGB}{230,45,45}

\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\begin{tabular}{l|l|l}
\Xhline{3\arrayrulewidth}
Transfer & To Future + Passive To Active & To Past + PP Removal \\ \hline
Source Sentence & \begin{tabular}[c]{@{}l@{}}NUM \% was risen by sales to NUM billion from NUM billion.\end{tabular} & \begin{tabular}[c]{@{}l@{}}the bond market was unmoved\\ by the economic statistics.
\end{tabular} \\ \hline
\modelshort & {\color{gg}sales will rise NUM \% to NUM billion from NUM billion.} & {\color{gg}the bond market is unmoved.} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Two examples of successful compositional transfers generated by \modelshort.\vspace{-4mm}}
\label{tab:comp_example}
\end{table*}

==> NAACL2021_Disentangling Text/tables/easy_full.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transfer & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\ \hline
\multirow{3}{*}{To Future Tense} & \textsc{GPT2} & 0.895 & 0.852 & 0.813 & \textbf{0.778} & \textbf{0.540} & 0.899 & 7.709 \\
 & \textsc{Seq2seq} & 0.527 & 0.368 & 0.261 & 0.188 & 0.173 & 0.531 & 1.525 \\
 & \textsc{RetrieveEdit} & \textbf{0.899} & \textbf{0.854} & \textbf{0.815} & \textbf{0.778} & 0.531 & \textbf{0.901} & \textbf{7.731} \\ \cline{2-9}
 & \textsc{Human} & 0.954 & 0.915 & 0.884 & 0.855 & 0.636 & 0.964 & 9.174 \\\hline
\multirow{3}{*}{To Past Tense} & \textsc{GPT2} & 0.836 & 0.776 & 0.722 & 0.674 & 0.484 & 0.842 & 6.700 \\
 & \textsc{Seq2seq} & 0.478 & 0.313 & 0.204 & 0.133 & 0.155 & 0.490 & 1.374 \\
 & \textsc{RetrieveEdit} & \textbf{0.935} & \textbf{0.903} & \textbf{0.873} & \textbf{0.847} & \textbf{0.606} & \textbf{0.933} & \textbf{8.358} \\ \cline{2-9}
 & \textsc{Human} & 0.974 & 0.957 & 0.939 & 0.916 & 0.709 & 0.982 & 9.549 \\ \hline
\multirow{3}{*}{To Present Tense} & \textsc{GPT2} & 0.754 & 0.663 & 0.586 & 0.524 & 0.412 & 0.772 & 5.293 \\
 & \textsc{Seq2seq} & 0.516 & 0.361 & 0.267 & 0.210 & 0.190 & 0.518 & 1.819 \\
 & \textsc{RetrieveEdit} & \textbf{0.909} & \textbf{0.870} & \textbf{0.830} & \textbf{0.793} & \textbf{0.599} & \textbf{0.916} & \textbf{7.987} \\ \cline{2-9}
 & \textsc{Human} & 0.969 & 0.952 & 0.936 & 0.918 & 0.745 & 0.979 & 9.501 \\\hline
 
 \multirow{3}{*}{ADJ or ADV Removal} & \textsc{GPT2} & 0.647 & 0.508 & 0.394 & 0.308 & 0.313 & 0.652 & 3.259 \\
 & \textsc{Seq2seq} & 0.450 & 0.274 & 0.172 & 0.112 & 0.140 & 0.469 & 1.171 \\
 & \textsc{RetrieveEdit} & \textbf{0.897} & \textbf{0.841} & \textbf{0.786} & \textbf{0.731} & \textbf{0.511} & \textbf{0.919} & \textbf{7.461}\\ \cline{2-9}
 & \textsc{Human} & 0.933 & 0.894 & 0.870 & 0.847 & 0.591 & 0.965 & 8.924 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Evaluation results on easy transfers.\vspace{-4mm}}
\label{tab:bas_full}
\end{table*}

==> NAACL2021_Disentangling Text/tables/hammingdistance.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}[t]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\centering
\footnotesize
\begin{tabular}{clc}
\Xhline{3\arrayrulewidth}
\multicolumn{1}{l}{Difficulty} & Transfer & Hamming \textcolor{gg}{$\downarrow$} \\ \hline
\multirow{4}{*}{Easy} & ADJ or ADV removal & $1.531$ \\
 & To Present tense & $2.318$ \\
 & To Past tense & $2.447$ \\
 & To Future tense & $3.341$ \\ \hline
\multirow{5}{*}{Medium} & Information addition & $3.729$ \\
 & PP removal & $4.079$ \\
 & PP back to front & $5.429$ \\
 & Substatement removal & $5.625$ \\
 & PP front to back & $6.235$ \\ \hline
\multirow{4}{*}{Hard} & Active to passive & $8.147$ \\
 & Passive to active & $8.817$ \\
 & Adjective emphasis & $8.846$ \\
 & Verb/Action emphasis & $11.614$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{\label{tab:ham} Average token-level Hamming distance between original and transferred sentences for all syntax, semantics and thematic transfers.\vspace{-2mm}}
\end{table}

==> NAACL2021_Disentangling Text/tables/hard_full.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transfer & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\ \hline
\multirow{3}{*}{Active To Passive} & \textsc{GPT2} & 0.476 & 0.329 & 0.238 & 0.189 & 0.216 & 0.464 & 1.820 \\
 & \textsc{Seq2seq} & 0.373 & 0.220 & 0.141 & 0.103 & 0.131 & 0.345 & 0.845 \\
 & \textsc{RetrieveEdit} & \textbf{0.681} & \textbf{0.598} & \textbf{0.503} & \textbf{0.427} & \textbf{0.383} & \textbf{0.663} & \textbf{4.535} \\\cline{2-9}
 & \textsc{Human} &  0.931 & 0.881 & 0.835 & 0.795 & 0.587 & 0.905 & 8.603 \\ \hline
\multirow{3}{*}{Passive To Active} & \textsc{GPT2} & 0.433 & 0.271 & 0.167 & 0.120 & 0.191 & 0.434 & 1.329 \\
 & \textsc{Seq2seq} & 0.339 & 0.214 & 0.160 & 0.132 & 0.126 & 0.331 & 1.062 \\
 & \textsc{RetrieveEdit} & \textbf{0.714} & \textbf{0.659} & \textbf{0.559} & \textbf{0.474} & \textbf{0.397} & \textbf{0.732} & \textbf{5.024} \\ \cline{2-9}
 & \textsc{Human} & 0.977 & 0.962 & 0.942 & 0.919 & 0.685 & 0.973 & 9.409 \\\hline
\multirow{3}{*}{Adjective Emphasis} & \textsc{GPT2} & 0.263 & 0.079 & 0.028 & 0.000 & 0.112 & 0.188 & 0.386 \\
 & \textsc{Seq2seq} & 0.187 & 0.058 & 0.018 & 0.000 & 0.059 & 0.179 & 0.141 \\
 & \textsc{RetrieveEdit} & \textbf{0.387} & \textbf{0.276} & \textbf{0.211} & \textbf{0.164} & \textbf{0.193} & \textbf{0.369} & \textbf{1.679} \\\cline{2-9}
 & \textsc{Human} & 0.834 & 0.753 & 0.679 & 0.611 & 0.522 & 0.811 & 6.796 \\ \hline
\multirow{3}{*}{Verb/Action Emphasis} & \textsc{GPT2} & 0.309 & 0.170 & 0.095 & 0.041 & 0.140 & 0.292 & 0.593 \\
 & \textsc{Seq2seq} & 0.289 & 0.127 & 0.066 & 0.038 & 0.098 & 0.275 & 0.300 \\
 & \textsc{RetrieveEdit} & \textbf{0.416} & \textbf{0.284} & \textbf{0.209} & \textbf{0.148} & \textbf{0.223} & \textbf{0.423} & \textbf{1.778}\\ \cline{2-9}
 & \textsc{Human} & 0.649 & 0.569 & 0.493 & 0.421 & 0.433 & 0.693 & 5.668 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on hard transfers. Thematic transfers are especially difficult for current models.\vspace{-4mm}}
\label{tab:bas3_full}
\end{table*}

==> NAACL2021_Disentangling Text/tables/hard_short.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transformation & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\ \hline
\multirow{3}{*}{Active To Passive} & \textsc{GPT2} & 0.476 & 0.329 & 0.238 & 0.189 & 0.216 & 0.464 & 1.820 \\
 & \textsc{Seq2seq} & 0.373 & 0.220 & 0.141 & 0.103 & 0.131 & 0.345 & 0.845 \\
 & \textsc{RetrieveEdit} & \textbf{0.681} & \textbf{0.598} & \textbf{0.503} & \textbf{0.427} & \textbf{0.383} & \textbf{0.663} & \textbf{4.535} \\ \hline
\multirow{3}{*}{Adjective Emphasis} & \textsc{GPT2} & 0.263 & 0.079 & 0.028 & 0.000 & 0.112 & 0.188 & 0.386 \\
 & \textsc{Seq2seq} & 0.187 & 0.058 & 0.018 & 0.000 & 0.059 & 0.179 & 0.141 \\
 & \textsc{RetrieveEdit} & \textbf{0.387} & \textbf{0.276} & \textbf{0.211} & \textbf{0.164} & \textbf{0.193} & \textbf{0.369} & \textbf{1.679} \\ \hline
\multirow{3}{*}{Verb/Action Emphasis} & \textsc{GPT2} & 0.309 & 0.170 & 0.095 & 0.041 & 0.140 & 0.292 & 0.593 \\
 & \textsc{Seq2seq} & 0.289 & 0.127 & 0.066 & 0.038 & 0.098 & 0.275 & 0.300 \\
 & \textsc{RetrieveEdit} & \textbf{0.416} & \textbf{0.284} & \textbf{0.209} & \textbf{0.148} & \textbf{0.223} & \textbf{0.423} & \textbf{1.778}\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on hard transfers. Thematic transfers are especially difficult for current models.\vspace{-4mm}}
\label{tab:bas3_short}
\end{table*}

==> NAACL2021_Disentangling Text/tables/human.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{6.0pt}
\centering
\footnotesize
\begin{tabular}{l|ccc}
\Xhline{3\arrayrulewidth}
& Clarity & Context & Style\\
\hline
\textsc{GPT2} & $1.60$ & $2.20$ & $\mathbf{4.05}$ \\
\textsc{Seq2seq} & $3.85$ & $1.45$ & $1.25$ \\
\textsc{RetrieveEdit} & $\mathbf{4.15}$ & $2.65$ & $2.20$ \\
\textsc{Human} & $\mathbf{4.70}$ & $\mathbf{4.45}$ & $\mathbf{5.00}$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Human evaluation of style transfer models trained on the Verb Emphasis task. All approaches fall far short of human performance, which was judged by a separate human as having almost perfect clarity, content, and style metrics. \textsc{GPT2} gets higher style scores while \textsc{RetrieveEdit} excels at grammar and content preservation.\vspace{-2mm}}
\label{human}
\end{table}

==> NAACL2021_Disentangling Text/tables/humanauteval.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.0pt}
\centering
\footnotesize
\begin{tabular}{lccc}
\Xhline{3\arrayrulewidth}
 & \multicolumn{1}{l}{Clarity} & \multicolumn{1}{l}{Content} & \multicolumn{1}{l}{Style} \\ \hline
Active To Passive & 4.93 & 5.00 & 4.87 \\
Passive To Active & 5.00 & 5.00 & 5.00 \\
To Future & 4.87 & 5.00 & 5.00 \\
To Present & 5.00 & 5.00 & 5.00 \\
To Past & 5.00 & 5.00 & 5.00 \\
PP Front To Back & 5.00 & 5.00 & 5.00 \\
PP Back To Front & 5.00 & 4.83 & 5.00 \\
ADJ/ADV Removal & 4.97 & 5.00 & 5.00 \\
PP Removal & 5.00 & 4.97 & 5.00 \\
Substatement Removal & 5.00 & 5.00 & 5.00 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{\label{tab:huaut}Human evaluations of randomly sampled automatically generated sentence transfers. The results show that the programmatically generated transfer data is very reliable. \vspace{-4mm}}

\end{table*}

==> NAACL2021_Disentangling Text/tables/humanfull.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{6.0pt}
\centering
\footnotesize
\begin{tabular}{llccc}
\Xhline{3\arrayrulewidth}
 &  & \multicolumn{1}{l}{Clarity} & \multicolumn{1}{l}{Content} & \multicolumn{1}{l}{Style} \\ \hline
\multirow{4}{*}{Active To Passive} & \textsc{GPT2} & 2.50 & 2.95 & 2.70 \\
 & \textsc{Seq2Seq} & 1.95 & 1.75 & 2.00 \\
 & \textsc{RetrieveEdit} & \textbf{4.05} & \textbf{3.65} & \textbf{4.10} \\ \cline{2-5} 
 & \textsc{Human} & 5.00 & 5.00 & 4.55 \\ \hline
\multirow{4}{*}{To Future} & \textsc{GPT2} & 4.65 & \textbf{4.85} & \textbf{4.80} \\
 & \textsc{Seq2Seq} & 2.05 & 2.20 & 3.25 \\
 & \textsc{RetrieveEdit} & \textbf{4.70} & 4.70 & 4.35 \\ \cline{2-5} 
 & \textsc{Human} & 5.00 & 5.00 & 5.00 \\ \hline
\multirow{4}{*}{ADJ/ADV Removal} & \textsc{GPT2} & 2.65 & 3.50 & \textbf{4.40} \\
 & \textsc{Seq2Seq} & 2.50 & 1.45 & 3.10 \\
 & \textsc{RetrieveEdit} & \textbf{4.65} & \textbf{4.45} & 4.25 \\ \cline{2-5} 
 & \textsc{Human} & 4.95 & 4.95 & 4.25 \\ \hline
\multirow{4}{*}{Substatement Removal} & \textsc{GPT2} & 3.05 & 3.15 & 3.95 \\
 & \textsc{Seq2Seq} & 3.30 & 2.05 & 3.75 \\
 & \textsc{RetrieveEdit} & \textbf{4.30} & \textbf{3.65} & \textbf{4.20} \\ \cline{2-5} 
 & \textsc{Human} & 5.00 & 5.00 & 3.55 \\ \hline
\multirow{4}{*}{Info Add} & \textsc{GPT2} & 2.15 & \textbf{2.55} & \textbf{3.05} \\
 & \textsc{Seq2Seq} & 2.70 & 1.35 & 1.60 \\
 & \textsc{RetrieveEdit} & \textbf{4.00} & \textbf{2.55} & 2.75 \\ \cline{2-5} 
 & \textsc{Human} & 5.00 & 4.80 & 4.70 \\ \hline
\multirow{4}{*}{ADJ emph} & \textsc{GPT2} & 1.30 & 2.65 & 2.85 \\
 & \textsc{Seq2Seq} & 2.65 & 1.05 & 1.00 \\
 & \textsc{RetrieveEdit} & \textbf{4.15} & \textbf{3.05} & \textbf{3.00} \\ \cline{2-5} 
 & \textsc{Human} & 4.55 & 4.75 & 4.75 \\ \hline
\multirow{4}{*}{VB emph} & \textsc{GPT2} & 1.60 & 2.20 & \textbf{4.05} \\
 & \textsc{Seq2Seq} & 3.85 & 1.45 & 1.25 \\
 & \textsc{RetrieveEdit} & \textbf{4.15} & \textbf{2.65} & 2.20 \\ \cline{2-5} 
 & \textsc{Human} & 4.70 & 4.45 & 5.00 \\ 
 
 \Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Human evaluation for single atomic style transfer on 7 selected transfers (the 7 transfers with BLEU scores appearing in main part of paper). The result shows that on harder transfers, all approaches fall short of human performance, and that \textsc{GPT2} excels at style while \textsc{RetrieveEdit} is better at grammar and content preservation.\vspace{-2mm}}
\label{humanfull}
\end{table}

==> NAACL2021_Disentangling Text/tables/med_full.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transfer & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\ \hline
\multirow{3}{*}{PP Front to Back} & \textsc{GPT2} & 0.398 & 0.210 & 0.081 & 0.001 & 0.184 & 0.406 & 0.886 \\
 & \textsc{Seq2seq} & 0.393 & 0.280 & 0.207 & 0.161 & 0.162 & 0.391 & 1.492 \\
 & \textsc{RetrieveEdit} & \textbf{0.541} & \textbf{0.423} & \textbf{0.301} & \textbf{0.176} & \textbf{0.247} & \textbf{0.547} & \textbf{2.536} \\ \cline{2-9}
 & \textsc{Human} & 0.965 & 0.959 & 0.952 & 0.945 & 0.690 & 0.970 & 9.671 \\ \hline
\multirow{3}{*}{PP Back to Front} & \textsc{GPT2} & 0.407 & 0.241 & 0.091 & 0.001 & 0.166 & 0.406 & 0.931 \\
 & \textsc{Seq2seq} & 0.298 & 0.157 & 0.090 & 0.060 & 0.112 & 0.284 & 0.606 \\
 & \textsc{RetrieveEdit} & \textbf{0.649} & \textbf{0.584} & \textbf{0.535} & \textbf{0.491} & \textbf{0.333} & \textbf{0.656} & \textbf{4.667} \\ \cline{2-9}
 & \textsc{Human} & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 10.000 \\ \hline
\multirow{3}{*}{PP Removal} & \textsc{GPT2} & 0.763 & 0.700 & 0.645 & 0.593 & 0.419 & 0.787 & 6.012 \\
 & \textsc{Seq2seq} & 0.330 & 0.195 & 0.121 & 0.081 & 0.112 & 0.363 & 1.004 \\
 & \textsc{RetrieveEdit} & \textbf{0.798} & \textbf{0.770} & \textbf{0.739} & \textbf{0.712} & \textbf{0.478} & \textbf{0.846} & \textbf{7.111} \\ \cline{2-9}
 & \textsc{Human} & 0.957 & 0.944 & 0.931 & 0.919 & 0.681 & 0.976 & 9.207 \\\hline
\multirow{3}{*}{Substatement Removal} & \textsc{GPT2} & 0.430 & 0.332 & 0.247 & 0.176 & 0.250 & 0.588 & 3.090 \\
 & \textsc{Seq2seq} & 0.317 & 0.192 & 0.110 & 0.001 & 0.100 & 0.368 & 1.041 \\
 & \textsc{RetrieveEdit} & \textbf{0.706} & \textbf{0.678} & \textbf{0.647} & \textbf{0.607} & \textbf{0.405} & \textbf{0.767} & \textbf{6.183} \\ \cline{2-9} 
 & \textsc{Human} & 0.731 & 0.720 & 0.705 & 0.685 & 0.607 & 0.788 & 7.691 \\ \hline
\multirow{3}{*}{Information Addition} & \textsc{GPT2} & 0.479 & 0.305 & 0.189 & 0.121 & 0.207 & 0.475 & 1.359 \\
 & \textsc{Seq2seq} & 0.345 & 0.180 & 0.094 & 0.053 & 0.098 & 0.335 & 0.632 \\
 & \textsc{RetrieveEdit} & \textbf{0.493} & \textbf{0.396} & \textbf{0.328} & \textbf{0.275} & \textbf{0.284} & \textbf{0.603} & \textbf{3.401} \\ \cline{2-9}
 & \textsc{Human} & 0.846 & 0.762 & 0.690 & 0.624 & 0.521 & 0.892 & 6.863 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Evaluation results on medium transfers. \textsc{Info Addition} is especially hard for current models.\vspace{-4mm}}
\label{tab:bas2_full}
\end{table*}

==> NAACL2021_Disentangling Text/tables/med_short.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transformation & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\ \hline
%\multirow{3}{*}{PP Front to Back} & \textsc{GPT2} & 0.398 & 0.210 & 0.081 & 0.001 & 0.184 & 0.406 & 0.886 \\
% & \textsc{Seq2seq} & 0.393 & 0.280 & 0.207 & 0.161 & 0.162 & 0.391 & 1.492 \\
% & \textsc{RetrieveEdit} & \textbf{0.541} & \textbf{0.423} & \textbf{0.301} & \textbf{0.176} & \textbf{0.247} & \textbf{0.547} & \textbf{2.536} \\ \hline
\multirow{3}{*}{Substatement Removal} & \textsc{GPT2} & 0.430 & 0.332 & 0.247 & 0.176 & 0.250 & 0.588 & 3.090 \\
 & \textsc{Seq2seq} & 0.317 & 0.192 & 0.110 & 0.001 & 0.100 & 0.368 & 1.041 \\
 & \textsc{RetrieveEdit} & \textbf{0.706} & \textbf{0.678} & \textbf{0.647} & \textbf{0.607} & \textbf{0.405} & \textbf{0.767} & \textbf{6.183} \\ \hline
\multirow{3}{*}{Information Addition} & \textsc{GPT2} & 0.479 & 0.305 & 0.189 & 0.121 & 0.207 & 0.475 & 1.359 \\
 & \textsc{Seq2seq} & 0.345 & 0.180 & 0.094 & 0.053 & 0.098 & 0.335 & 0.632 \\
 & \textsc{RetrieveEdit} & \textbf{0.493} & \textbf{0.396} & \textbf{0.328} & \textbf{0.275} & \textbf{0.284} & \textbf{0.603} & \textbf{3.401} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Evaluation results on medium transfers. \textsc{Info Addition} is especially hard for current models.\vspace{-4mm}}
\label{tab:bas2_short}
\end{table*}

==> NAACL2021_Disentangling Text/tables/params.tex <==
\begin{table}[]
\fontsize{9}{11}\selectfont
\centering

\setlength\tabcolsep{3.5pt}
\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{10}{*}{\textsc{GPT}}
& pretrained model & GPT2 (small) with LM head \\
& pretrained encoder/decoder & GPT2 (small) \\
& batchsize & $20$ \\
& optimizer & RMSprop \\
& initial learning rate & $2e-5$ \\
& \#turns to half learning rate & $15$\\
& evaluate every \#iterations & $1$\\
& weight decay & $0.015$ \\
& teacher force ratio & $1.0$ \\
& max iterations & $60$\\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{10}{*}{\modelshort~and \textsc{\modelshort-zero}}
& pretrained model & GPT2 (small) with LM head \\
& pretrained encoder/decoder & GPT2 (small) \\
& batchsize & $20$ \\
& optimizer & RMSprop \\
& initial learning rate & $2e-5$ \\
& \#turns to half learning rate & $5$\\
& evaluate every \#iterations & $1$\\
& weight decay & $0.015$ \\
& teacher force ratio & $1.0$ \\
& max iterations & $30$\\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{12}{*}{\textsc{Seq2seq}}
& encoder GRU hidden size & $256$ \\
& decoder GRU hidden size & $256$ \\
& attention size & $256$ \\
& word embedding size & $256$ \\
& batchsize & $1$ \\
& optimizer & SGD \\
& initial learning rate & $1e-2$ \\
& \#turns to half learning rate & $5000$ \\
& evaluate every \#iterations & $1000$\\
& weight decay & $0.015$ \\
& teacher force ratio & $0.9$ \\
& max iterations & $185000$\\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l | c | c}
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{13}{*}{\textsc{RetrieveEdit}}
& encoder layers & $2$ \\
& decoder layers & $4$ \\
& hidden size & $256$ \\
& agenda size & $256$ \\
& attention size & $256$ \\
& word embedding size & $300$ \\
& batchsize & $16$ \\
& VAE-kappa & $500$ \\
& ident\_pr & $0.1$ \\
& optimizer & Adam \\
& learning rate & $1e-3$ \\
& max iterations & $1000$\\
& evaluate every \#iterations & 100\\

\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-0mm}
\caption{Table of hyperparameters for all models in all experiments respectively. Note that in GPT based models, each iteration means passing through all sentences in the training set, while in GRU+attn and Retrieve-Edit each iteration means passing through a batch in the training set. Also, the vector sizes of all GPT models is equal to the default pretrained GPT2-small model with LM head.\vspace{-2mm}}
\label{hyperparams}
\end{table}

==> NAACL2021_Disentangling Text/tables/res_short.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\vspace{-6mm}
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
\textbf{Easy} Transfers & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\
\hline
\multirow{4}{*}{To Future Tense} & \textsc{GPT2} & 0.895 & 0.852 & 0.813 & \textbf{0.778} & \textbf{0.540} & 0.899 & 7.709 \\
 & \textsc{Seq2seq} & 0.527 & 0.368 & 0.261 & 0.188 & 0.173 & 0.531 & 1.525 \\
 & \textsc{RetrieveEdit} & \textbf{0.899} & \textbf{0.854} & \textbf{0.815} & \textbf{0.778} & 0.531 & \textbf{0.901} & \textbf{7.731} \\ \cline{2-9}
 & \textsc{Human} & 0.954 & 0.915 & 0.884 & 0.855 & 0.636 & 0.964 & 9.174 \\
 \hline
\multirow{4}{*}{ADJ or ADV Removal} & \textsc{GPT2} & 0.647 & 0.508 & 0.394 & 0.308 & 0.313 & 0.652 & 3.259 \\
 & \textsc{Seq2seq} & 0.450 & 0.274 & 0.172 & 0.112 & 0.140 & 0.469 & 1.171 \\
 & \textsc{RetrieveEdit} & \textbf{0.897} & \textbf{0.841} & \textbf{0.786} & \textbf{0.731} & \textbf{0.511} & \textbf{0.919} & \textbf{7.461}\\ \cline{2-9}
 & \textsc{Human} & 0.933 & 0.894 & 0.870 & 0.847 & 0.591 & 0.965 & 8.924 \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
\textbf{Medium} Transfers & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\
 \hline
%\multirow{3}{*}{PP Front to Back} & \textsc{GPT2} & 0.398 & 0.210 & 0.081 & 0.001 & 0.184 & 0.406 & 0.886 \\
% & \textsc{Seq2seq} & 0.393 & 0.280 & 0.207 & 0.161 & 0.162 & 0.391 & 1.492 \\
% & \textsc{RetrieveEdit} & \textbf{0.541} & \textbf{0.423} & \textbf{0.301} & \textbf{0.176} & \textbf{0.247} & \textbf{0.547} & \textbf{2.536} \\ \hline
\multirow{4}{*}{Substatement Removal} & \textsc{GPT2} & 0.430 & 0.332 & 0.247 & 0.176 & 0.250 & 0.588 & 3.090 \\
 & \textsc{Seq2seq} & 0.317 & 0.192 & 0.110 & 0.001 & 0.100 & 0.368 & 1.041 \\
 & \textsc{RetrieveEdit} & \textbf{0.706} & \textbf{0.678} & \textbf{0.647} & \textbf{0.607} & \textbf{0.405} & \textbf{0.767} & \textbf{6.183} \\ \cline{2-9} 
 & \textsc{Human} & 0.731 & 0.720 & 0.705 & 0.685 & 0.607 & 0.788 & 7.691 \\
 \hline
\multirow{4}{*}{Information Addition} & \textsc{GPT2} & 0.479 & 0.305 & 0.189 & 0.121 & 0.207 & 0.475 & 1.359 \\
 & \textsc{Seq2seq} & 0.345 & 0.180 & 0.094 & 0.053 & 0.098 & 0.335 & 0.632 \\
 & \textsc{RetrieveEdit} & \textbf{0.493} & \textbf{0.396} & \textbf{0.328} & \textbf{0.275} & \textbf{0.284} & \textbf{0.603} & \textbf{3.401} \\ \cline{2-9}
 & \textsc{Human} & 0.846 & 0.762 & 0.690 & 0.624 & 0.521 & 0.892 & 6.863 \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
\textbf{Hard} Transfers & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\ \hline
\multirow{4}{*}{Active To Passive} & \textsc{GPT2} & 0.476 & 0.329 & 0.238 & 0.189 & 0.216 & 0.464 & 1.820 \\
 & \textsc{Seq2seq} & 0.373 & 0.220 & 0.141 & 0.103 & 0.131 & 0.345 & 0.845 \\
 & \textsc{RetrieveEdit} & \textbf{0.681} & \textbf{0.598} & \textbf{0.503} & \textbf{0.427} & \textbf{0.383} & \textbf{0.663} & \textbf{4.535} \\ \cline{2-9}
 & \textsc{Human} &  0.931 & 0.881 & 0.835 & 0.795 & 0.587 & 0.905 & 8.603 \\
 \hline
\multirow{4}{*}{Adjective Emphasis} & \textsc{GPT2} & 0.263 & 0.079 & 0.028 & 0.000 & 0.112 & 0.188 & 0.386 \\
 & \textsc{Seq2seq} & 0.187 & 0.058 & 0.018 & 0.000 & 0.059 & 0.179 & 0.141 \\
 & \textsc{RetrieveEdit} & \textbf{0.387} & \textbf{0.276} & \textbf{0.211} & \textbf{0.164} & \textbf{0.193} & \textbf{0.369} & \textbf{1.679} \\ \cline{2-9}
 & \textsc{Human} & 0.834 & 0.753 & 0.679 & 0.611 & 0.522 & 0.811 & 6.796 \\
 \hline
\multirow{4}{*}{Verb/Action Emphasis} & \textsc{GPT2} & 0.309 & 0.170 & 0.095 & 0.041 & 0.140 & 0.292 & 0.593 \\
 & \textsc{Seq2seq} & 0.289 & 0.127 & 0.066 & 0.038 & 0.098 & 0.275 & 0.300 \\
 & \textsc{RetrieveEdit} & \textbf{0.416} & \textbf{0.284} & \textbf{0.209} & \textbf{0.148} & \textbf{0.223} & \textbf{0.423} & \textbf{1.778}\\ \cline{2-9}
 & \textsc{Human} & 0.649 & 0.569 & 0.493 & 0.421 & 0.433 & 0.693 & 5.668 \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\caption{Evaluation results on easy (top), medium (middle), and hard (bottom) transfers. {Info Addition} and thematic transfers are especially difficult for current models.\vspace{-4mm}}
\label{tab:bas_short}
\end{table*}

==> NAACL2021_Disentangling Text/tables/single_full.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transfer & Model & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & METEOR & ROUGE\_L & CiDER \\ \hline
To Future Tense & \textsc{GPT2} & \textbf{0.895} & \textbf{0.851} & \textbf{0.812} & \textbf{0.777} & \textbf{0.539} & \textbf{0.898} & \textbf{7.708} \\
 & \modelshort\ (TV) & 0.727 & 0.614 & 0.614 & 0.450 & 0.362 & 0.731 & 4.386 \\
 & \modelshort\ (TP) & 0.810 & 0.731 & 0.663 & 0.606 & 0.446 & 0.818 & 6.026 \\
 \hline
\multirow{3}{*}{To Past Tense} & \textsc{GPT2} & \textbf{0.835} & \textbf{0.776} & \textbf{0.721} & \textbf{0.673} & 0.484 & \textbf{0.842} & 6.699 \\ 
 & \modelshort\ (TV) & 0.694 & 0.586 & 0.494 & 0.420 & 0.353 & 0.700 & 4.051 \\
 & \modelshort\ (TP) & 0.834 & 0.771 & 0.718 & 0.672 & \textbf{0.486} & 0.841 & \textbf{6.704} \\
 \hline
\multirow{3}{*}{To Present Tense} & \textsc{GPT2} & 0.753 & 0.662 & 0.586 & 0.523 & 0.412 & 0.772 & 5.293 \\
 & \modelshort\ (TV) & 0.733 & 0.635 & 0.553 & 0.488 & 0.387 & 0.744 & 4.742 \\
 & \modelshort\ (TP) & \textbf{0.826} & \textbf{0.755} & \textbf{0.691} & \textbf{0.637} & \textbf{0.491} & \textbf{0.831} & \textbf{6.315} \\
 \hline
\multirow{2}{*}{ActiveToPassive} & \textsc{GPT2} & \textbf{0.475} & \textbf{0.329} & \textbf{0.238} & \textbf{0.189} & 0.216 & \textbf{0.463} & \textbf{1.820} \\
 & \modelshort\ (TV) & 0.472 & 0.324 & 0.232 & 0.179 & \textbf{0.216} & 0.454 & 1.790 \\
 \hline
\multirow{2}{*}{PassiveToActive} & \textsc{GPT2} & 0.433 & 0.271 & 0.167 & 0.120 & 0.191 & 0.434 & 1.329 \\
 & \modelshort\ (TV) & \textbf{0.506} & \textbf{0.345} & \textbf{0.243} & \textbf{0.184} & \textbf{0.229} & \textbf{0.505} & \textbf{1.958} \\
 \hline
\multirow{2}{*}{PP Removal} & \textsc{GPT2} & \textbf{0.763} & \textbf{0.700} & \textbf{0.645} & \textbf{0.593} & 0.419 & \textbf{0.786} & \textbf{6.011} \\
 & \modelshort\ (TP) & 0.760 & 0.698 & 0.639 & 0.585 & \textbf{0.420} & 0.772 & 5.783 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Comparing single transfer performances between \modelshort \ and \textsc{GPT2} baselines (where TV indicates the \modelshort\ is trained on Tense+Voice dataset and TP indicates the \modelshort\ is trained on Tense+PP Removal dataset). The result shows that \modelshort\ can perform multiple single style transfers with similar performance to \textsc{GPT2} trained specifically for that one transfer, and sometimes even outperforms \textsc{GPT2}.\vspace{-4mm}}
\label{tab:single_full}
\end{table*}

==> NAACL2021_Disentangling Text/tables/single_short.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transfer & Model & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & METEOR & ROUGE\_L & CiDER \\ \hline
\multirow{3}{*}{To Present Tense} & \textsc{GPT2} & 0.753 & 0.662 & 0.586 & 0.523 & 0.412 & 0.772 & 5.293 \\
 & \modelshort\ (TV) & 0.733 & 0.635 & 0.553 & 0.488 & 0.387 & 0.744 & 4.742 \\
 & \modelshort\ (TP) & \textbf{0.826} & \textbf{0.755} & \textbf{0.691} & \textbf{0.637} & \textbf{0.491} & \textbf{0.831} & \textbf{6.315} \\
 \hline
\multirow{2}{*}{PassiveToActive} & \textsc{GPT2} & 0.433 & 0.271 & 0.167 & 0.120 & 0.191 & 0.434 & 1.329 \\
 & \modelshort\ (TV) & \textbf{0.506} & \textbf{0.345} & \textbf{0.243} & \textbf{0.184} & \textbf{0.229} & \textbf{0.505} & \textbf{1.958} \\
 \hline
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Comparing \modelshort\ trained on compositional data (TV: Tense+Voice, TP: Tense+PP removal) with \textsc{GPT2} models. Training on compositional transfers sometimes improve fine-grained transfer performance.\vspace{-2mm}}
\label{tab:single_short}
\end{table*}

==> NAACL2021_Disentangling Text/tables/tenseapstats.tex <==
\begin{table}[t]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.0pt}
\centering
\footnotesize
\begin{tabular}{l|ccc}
\Xhline{3\arrayrulewidth}
& \begin{tabular}[c]{@{}l@{}}No Voice \\ Change (0)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Active To \\ Passive (1)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Passive To \\ Active (2)\end{tabular} \\
\hline
No Tense Change (0) & $2808$ & $2808$ & $2808$ \\
To Future Tense (1) & $5294$ & $2647$ & $2647$ \\
To Past Tense (2) & $2077$ & $656$ & $1421$ \\
To Present Tense (3) & $3304$ & $1536$ & $1768$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Number of sentence pairs for each composition of tense change and voice change in the generated compositional dataset.\vspace{-2mm}}
\label{compAP}
\end{table}

% Number of parallel pairs of sentences for each composition of tense change and voice change in the generated compositional dataset

==> tables/baselineresults.tex <==
\footnotesize
\begin{tabular}{|l|l|r|r|r|r|r|r|r|}
\hline
Baseline Model & Transformation & \multicolumn{1}{l|}{BLEU-1} & \multicolumn{1}{l|}{BLEU-2} & \multicolumn{1}{l|}{BLEU-3} & \multicolumn{1}{l|}{BLEU-4} & \multicolumn{1}{l|}{METEOR} & \multicolumn{1}{l|}{ROUGE\_L} & \multicolumn{1}{l|}{CiDER} \\ \hline
\multirow{13}{*}{GPT Baseline} & To Future Tense & 0.8954 & 0.8519 & 0.8127 & 0.7776 & 0.5399 & 0.8987 & 7.7087 \\ \cline{2-9} 
 & To Present Tense & 0.8357 & 0.7762 & 0.7219 & 0.6738 & 0.484 & 0.8422 & 6.6996 \\ \cline{2-9} 
 & To Past tense & 0.7539 & 0.6625 & 0.5862 & 0.5237 & 0.4121 & 0.7722 & 5.2932 \\ \cline{2-9} 
 & Active to Passive & 0.4756 & 0.3293 & 0.2382 & 0.189 & 0.216 & 0.4635 & 1.8209 \\ \cline{2-9} 
 & Passive to active & 0.4325 & 0.2709 & 0.1672 & 0.1203 & 0.1908 & 0.4344 & 1.3287 \\ \cline{2-9} 
 & PP Front to Back & 0.3976 & 0.2095 & 0.0808 & 0.0006 & 0.1836 & 0.4057 & 0.886 \\ \cline{2-9} 
 & PP back to Front & 0.4065 & 0.2413 & 0.0912 & 0.0007 & 0.1659 & 0.4061 & 0.9306 \\ \cline{2-9} 
 & ADJ or ADV Removal & 0.6471 & 0.508 & 0.3941 & 0.3084 & 0.3125 & 0.6523 & 3.2589 \\ \cline{2-9} 
 & PP Removal & 0.7631 & 0.7004 & 0.6451 & 0.593 & 0.4192 & 0.7867 & 6.0119 \\ \cline{2-9} 
 & Substatement Removal & 0.4303 & 0.3316 & 0.2474 & 0.1757 & 0.2498 & 0.5881 & 3.0894 \\ \cline{2-9} 
 & Information Addition & 0.4793 & 0.3048 & 0.1891 & 0.1205 & 0.2074 & 0.4746 & 1.3588 \\ \cline{2-9} 
 & Adjective Emphasis & 0.2629 & 0.0793 & 0.0282 & 0.0003 & 0.1122 & 0.1884 & 0.3863 \\ \cline{2-9} 
 & Verb/Action Emphasis & 0.3087 & 0.1697 & 0.0949 & 0.0405 & 0.1399 & 0.2921 & 0.5925 \\ \hline
\multirow{13}{*}{GRU attn} & To Future Tense & 0.5271 & 0.3675 & 0.2609 & 0.1884 & 0.1727 & 0.5309 & 1.5253 \\ \cline{2-9} 
 & To Present Tense & 0.4784 & 0.3129 & 0.2043 & 0.1328 & 0.1552 & 0.4898 & 1.3735 \\ \cline{2-9} 
 & To Past tense & 0.516 & 0.3605 & 0.2674 & 0.2101 & 0.1899 & 0.5178 & 1.8185 \\ \cline{2-9} 
 & Active to Passive & 0.3725 & 0.2199 & 0.1414 & 0.103 & 0.1308 & 0.3451 & 0.8446 \\ \cline{2-9} 
 & Passive to active & 0.3394 & 0.2137 & 0.16 & 0.1315 & 0.1262 & 0.3314 & 1.0615 \\ \cline{2-9} 
 & PP Front to Back & 0.3928 & 0.2802 & 0.2071 & 0.1607 & 0.1618 & 0.3914 & 1.4918 \\ \cline{2-9} 
 & PP back to Front & 0.2978 & 0.1572 & 0.0904 & 0.0595 & 0.1123 & 0.2836 & 0.6057 \\ \cline{2-9} 
 & ADJ or ADV Removal & 0.4497 & 0.2735 & 0.1723 & 0.1118 & 0.1398 & 0.4688 & 1.1711 \\ \cline{2-9} 
 & PP Removal & 0.3303 & 0.1949 & 0.1212 & 0.0814 & 0.1124 & 0.3634 & 1.0036 \\ \cline{2-9} 
 & Substatement Removal & 0.3165 & 0.1924 & 0.1096 & 0.0009 & 0.1004 & 0.3678 & 1.0409 \\ \cline{2-9} 
 & Information Addition & 0.345 & 0.1804 & 0.094 & 0.0527 & 0.0983 & 0.335 & 0.6315 \\ \cline{2-9} 
 & Adjective Emphasis & 0.1873 & 0.0581 & 0.0184 & 0.0002 & 0.0593 & 0.1794 & 0.1414 \\ \cline{2-9} 
 & Verb/Action Emphasis & 0.2885 & 0.1268 & 0.0656 & 0.0379 & 0.0982 & 0.2748 & 0.3003 \\ \hline
\multirow{13}{*}{RetrieveEdit} & To Future Tense & 0.8992 & 0.8536 & 0.8145 & 0.7783 & 0.531 & 0.9013 & 7.7309 \\ \cline{2-9} 
 & To Present Tense & 0.9352 & 0.9031 & 0.8731 & 0.8474 & 0.6062 & 0.9328 & 8.3577 \\ \cline{2-9} 
 & To Past tense & 0.9094 & 0.8702 & 0.8302 & 0.7926 & 0.5986 & 0.9156 & 7.9874 \\ \cline{2-9} 
 & Active to Passive & 0.6809 & 0.5981 & 0.5031 & 0.4273 & 0.3827 & 0.6629 & 4.5351 \\ \cline{2-9} 
 & Passive to active & 0.7143 & 0.6587 & 0.5592 & 0.4744 & 0.397 & 0.7317 & 5.024 \\ \cline{2-9} 
 & PP Front to Back & 0.5408 & 0.4226 & 0.3009 & 0.1763 & 0.2474 & 0.5474 & 2.5362 \\ \cline{2-9} 
 & PP back to Front & 0.6486 & 0.5842 & 0.5353 & 0.4914 & 0.3333 & 0.6563 & 4.6667 \\ \cline{2-9} 
 & ADJ or ADV Removal & 0.8972 & 0.8408 & 0.7855 & 0.7307 & 0.5109 & 0.9185 & 7.4607 \\ \cline{2-9} 
 & PP Removal & 0.798 & 0.7704 & 0.7392 & 0.7117 & 0.4778 & 0.8455 & 7.1105 \\ \cline{2-9} 
 & Substatement Removal & 0.7056 & 0.6783 & 0.6474 & 0.6068 & 0.4053 & 0.7671 & 6.183 \\ \cline{2-9} 
 & Information Addition & 0.4928 & 0.3959 & 0.3282 & 0.2746 & 0.2841 & 0.6028 & 3.4011 \\ \cline{2-9} 
 & Adjective Emphasis & 0.3866 & 0.276 & 0.2106 & 0.1637 & 0.1933 & 0.369 & 1.6793 \\ \cline{2-9} 
 & Verb/Action Emphasis & 0.4162 & 0.2844 & 0.2091 & 0.1483 & 0.2229 & 0.4234 & 1.7782 \\ \hline
\end{tabular}

==> tables/hard_short.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transformation & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\ \hline
\multirow{3}{*}{Active To Passive} & \textsc{GPT2} & 0.476 & 0.329 & 0.238 & 0.189 & 0.216 & 0.464 & 1.820 \\
 & \textsc{Seq2seq} & 0.373 & 0.220 & 0.141 & 0.103 & 0.131 & 0.345 & 0.845 \\
 & \textsc{RetrieveEdit} & \textbf{0.681} & \textbf{0.598} & \textbf{0.503} & \textbf{0.427} & \textbf{0.383} & \textbf{0.663} & \textbf{4.535} \\ \hline
\multirow{3}{*}{Adjective Emphasis} & \textsc{GPT2} & 0.263 & 0.079 & 0.028 & 0.000 & 0.112 & 0.188 & 0.386 \\
 & \textsc{Seq2seq} & 0.187 & 0.058 & 0.018 & 0.000 & 0.059 & 0.179 & 0.141 \\
 & \textsc{RetrieveEdit} & \textbf{0.387} & \textbf{0.276} & \textbf{0.211} & \textbf{0.164} & \textbf{0.193} & \textbf{0.369} & \textbf{1.679} \\ \hline
\multirow{3}{*}{Verb/Action Emphasis} & \textsc{GPT2} & 0.309 & 0.170 & 0.095 & 0.041 & 0.140 & 0.292 & 0.593 \\
 & \textsc{Seq2seq} & 0.289 & 0.127 & 0.066 & 0.038 & 0.098 & 0.275 & 0.300 \\
 & \textsc{RetrieveEdit} & \textbf{0.416} & \textbf{0.284} & \textbf{0.209} & \textbf{0.148} & \textbf{0.223} & \textbf{0.423} & \textbf{1.778}\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on hard transfers. Thematic transfers are especially difficult for current models.\vspace{-4mm}}
\label{tab:bas3_short}
\end{table*}

==> tables/med_short.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{5.0pt}
\centering
\footnotesize
\begin{tabular}{llccccccc}
\Xhline{3\arrayrulewidth}
Transformation & Baseline Model & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{ROUGE\_L} & \multicolumn{1}{l}{CiDER} \\ \hline
%\multirow{3}{*}{PP Front to Back} & \textsc{GPT2} & 0.398 & 0.210 & 0.081 & 0.001 & 0.184 & 0.406 & 0.886 \\
% & \textsc{Seq2seq} & 0.393 & 0.280 & 0.207 & 0.161 & 0.162 & 0.391 & 1.492 \\
% & \textsc{RetrieveEdit} & \textbf{0.541} & \textbf{0.423} & \textbf{0.301} & \textbf{0.176} & \textbf{0.247} & \textbf{0.547} & \textbf{2.536} \\ \hline
\multirow{3}{*}{Substatement Removal} & \textsc{GPT2} & 0.430 & 0.332 & 0.247 & 0.176 & 0.250 & 0.588 & 3.090 \\
 & \textsc{Seq2seq} & 0.317 & 0.192 & 0.110 & 0.001 & 0.100 & 0.368 & 1.041 \\
 & \textsc{RetrieveEdit} & \textbf{0.706} & \textbf{0.678} & \textbf{0.647} & \textbf{0.607} & \textbf{0.405} & \textbf{0.767} & \textbf{6.183} \\ \hline
\multirow{3}{*}{Information Addition} & \textsc{GPT2} & 0.479 & 0.305 & 0.189 & 0.121 & 0.207 & 0.475 & 1.359 \\
 & \textsc{Seq2seq} & 0.345 & 0.180 & 0.094 & 0.053 & 0.098 & 0.335 & 0.632 \\
 & \textsc{RetrieveEdit} & \textbf{0.493} & \textbf{0.396} & \textbf{0.328} & \textbf{0.275} & \textbf{0.284} & \textbf{0.603} & \textbf{3.401} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Evaluation results on medium transfers. \textsc{Info Addition} is especially hard for current models.\vspace{-4mm}}
\label{tab:bas2_short}
\end{table*}
